Proof-of-Execution: Reaching Consensus through Fault-Tolerant Speculation

Multi-party data management and blockchain systems require data sharing among participants. To provide resilient and consistent data sharing, transactions engines rely on Byzantine FaultTolerant consensus (BFT), which enables operations during failures and malicious behavior. Unfortunately, existing BFT protocols are unsuitable for high-throughput applications due to their high computational costs, high communication costs, high client latencies, and/or reliance on twin-paths and non-faulty clients. In this paper, we present the Proof-of-Execution consensus protocol (PoE) that alleviates these challenges. At the core of PoE are out-of-order processing and speculative execution, which allow PoE to execute transactions before consensus is reached among the replicas. With these techniques, PoE manages to reduce the costs of BFT in normal cases, while guaranteeing reliable consensus for clients in all cases. We envision the use of PoE in high-throughput multi-party data-management and blockchain systems. To validate this vision, we implement PoE in our efficient ResilientDB fabric and extensively evaluate PoE against several state-of-the-art BFT protocols. Our evaluation showcases that PoE achieves up-to-80% higher throughputs than existing BFT protocols in the presence of failures.

==> discuss.tex <==
\subsection{Out-of-Order Message Processing}
\label{s:discuss}
Single-primary protocols like \pbft{}, \SBFT{}, and \PoE{}, offer a unique opportunity of pipelining and 
parallelizing multiple $\MName{Propose}$ messages. 
In these protocols, the primary replica need not wait for one consensus to finish before starting the consensus 
for next request.
This allows replicas to process messages {\bf \em out-of-order} while they continue executing transactions 
in the sequence-order.
For example, \pbft{} allows such an optimization by defining an active-set of 
sequence numbers bounded by {\em high-watermark} and {\em low-watermark}~\cite{pbftj,pbftthesis}. 
These watermarks are increased as the system progresses.
 
In case of \PoE{}, notice that a backup replica only accepts $k$-th proposal from the primary if it had not 
previously supported another $k$-th proposal (Figure~\ref{fig:pa}, Line~\ref{fig:k-proposal}).
Further, a replica only executes a $k$-th request if it has executed requests for all the previous rounds 
(Figure~\ref{fig:pa}, Line~\ref{fig:pa:exec}).
Hence, the primary need not wait for the consensus of $k$-th request to complete before sending out $\MName{Propose}$
message for $(k+1)$-th request.
%
In case of rotating primary protocols such as \hotstuff{}, this out-of-ordering is not feasible. 
We illustrate this in more detail in Section~\ref{ss:other}.




